A Random Network Model for the Analysis of Blockchain Designs with Communication Delay

This paper proposes a random network model for blockchains, a distributed hierarchical data structure of blocks that has found several applications in various industries. The model is parametric on two probability distribution functions governing block production and communication delay, which are key to capture the complexity of the mechanism used to synchronize the many distributed local copies of a blockchain. The proposed model is equipped with simulation algorithms for both bounded and unbounded number of distributed copies of the blockchain. They are used to study fast blockchain systems, i.e., blockchains in which the average time of block production can match the average time of message broadcasting used for blockchain synchronization. In particular, the model and the algorithms are useful to understand efficiency criteria associated with fast blockchains for identifying, e.g., when increasing the block production will have negative impact on the stability of the distributed data structure given the network's broadcast delay.

==> old/algo.tex <==
\section{Algorithms}
\label{sec.algo}


\subsection{Network simulation algorithm}

The first and most intuitive algorithm for simulating blockchain growth is the
network simulation. It simulates the production of $n$ blocks by $m$ workers
in the network, each with its own sequence of blocks.

\begin{lstlisting}[language=Python]
def NetworkSim(m, n, T, L):
    t, maxh = 0, 0
    R = [[] for w in range(m)]
    for w in range(m):
        R[i].append((0, 0))
    for step in range(n):
        t = t + T()
        w = randrange(m)
        h = max(h for (tr, h) in R[w] if tr <= t)
        for x in range(m):
            trecv = t + L() if w != x else t
            R[x].append((trecv, 1 + h))
        maxh = max(maxh, 1 + h)
    return maxh / n
\end{lstlisting}

The algorithm has an runtime complexity of $O(m\cdot n)$, and a memory
complexity of also $O(m\cdot n)$. This is very limiting given that we are
mainly interested in producing several ($n>>0$) blocks in highly
distributed networks ($m\to \infty$).


\subsection{Infinite workers simulation algorithm}

In order to speed-up the network simulation, the following approximation
algorithm was proposed. It has a memory complexity of $O(n)$ and an average
runtime complexity of $O(n\cdot \bar{T}/\bar{L})$.

\begin{lstlisting}[language=Python]
def InfWorkersSim(n, T, L):
    t = 0
    maxh = 0
    prod = [(0, 0, 0)]
    for step in range(n):
        t = t + T()
        h, i = 0, len(prod) - 1
        while i >= 0 and prod[i][2] > h:
            if prod[i][0] < t + L():
              h = max(h, prod[i][1])
            i = i - 1
        maxh = max(maxh, h + 1)
        prod.append((t, h + 1, maxh))
    return maxh / n
\end{lstlisting}

An equivalent version of this algorithm that is slower $O(n^2)$ but easier to
analyze is shown below.

\begin{lstlisting}[language=Python]
def InfWorkersSim(n, T, L):
    t = 0
    maxh = 0
    prod = [(0, 0)]
    seen = lambda tx: tx <= t - L() or tx == 0
    for step in range(n):
        t = t + T()
        h = max(hx for (tx, hx) in prod if seen(tx))
        prod.append((t, h+1))
        maxh = max(maxh, h+1)
    return maxh / n
\end{lstlisting}


==> old/intro.tex <==
\section{Introduction}
\label{sec.intro}

Blockchain systems are becoming very popular these days and are expanding into
areas different from cryptocurrencies such as decentralized protection of
personal data, digital property, Internet of things and
healthcare\cite{karafiloski2017blockchain}. These systems rely on a public
ledger called the blockchain.

A blockchain is a decentralized append-only datastructure. It is a linear set
of blocks, shared between several nodes in a network. These nodes are called
miners or workers, beacuse they are responsible of working on top of the
blockchain to extend it further with new blocks. However, since the
datastructure is decentralized, each worker possesses its own copy of the
blockchain, and this means that two workers might be working on top of
different blocks if they are not synchronized.

If several workers extend different versions of the blockchain, the network as
a whole will eventually select only one of them by means of a consensus
protocol; the others will be discarded, and so will the information or
transactions they carried. The only rule of the consensus protocol is to work
on top of the largest blockchain, and in case of ties, on the one whose last
produced block was seen earliest. This protocol guarantees stability as long
as the task of producing blocks stays hard to achieve, which is what is known
in the literature as proof of work.

This scenario is not present very often in slow blockchain systems such as
bitcoin, because the time between consecutive blocks (10 min. in average) is
usually enough for the workers to synchronize. But it does happen, and it was
shown\cite{decker2013information} that the theoretical fork-rate for bitcoin
was approximately 1.78\% in 2013.

In fast blockchain systems, on the other hand, the scenario is by definition
very common and the unstability is therefore higher. This implies not only a
higher rate of discarded blocks, but also a higher chance of performing
double-spend attacks, as shown in \cite{kiayias2015speed}. Unlike their work,
which focuses on the trade-off between speed and security, this paper assumes
the best case security scenario (no attackers at all), and still analyses the
consequences of having short waiting times between blocks, yielding a
speed-stability trade-off.

This paper is organized as follows...

==> old/model.tex <==
\section{Model}
\label{sec.model}

The proposed model considers many workers with similar computing power that
produce blocks in a proof-of-work fashion following the standard protocol and
communicating in a network to extend their blockchains. The time between
consecutive blocks is denoted with the random variable $T$, and the
communication delay between any pair of workers in the network is assumed to
follow a distribution given by the \emph{lag} random variable $L$.

There is one synchronization detail that is not covered by the standard
protocol, and which plays an important role in fast systems, namely, what
happens when a block is received but its previous has not been received yet.
Since there is no defacto standard for this scenario, this model assumes the
simplest one: \emph{messages of newly created blocks include enough
information about their previous blocks, so that no retransmission is required
to fill block gaps}, or equivalently, these retransmission times are included
in the \emph{lag} variable.

Under these constraints, the two inputs for the model are $T$ and $L$, and the
blockchain growth can be simulated by repeating the following procedure:

\begin{enumerate}
  \item A random worker produces the next block in $T$ seconds. The block
  extends the longest branch the worker is aware of (initially just the origin
  block).
  \item The block is broadcasted and will reach the other workers in $L$
  seconds, being $L$ sampled separately for each worker.
\end{enumerate}

Once the procedure has been repeated enough times, several metrics can be
extracted from the blockchain tree. In particular, $p$, which is the length of
the longest branch divided by the total number of produced blocks is important
because it can be used to determine many other metrics.

\begin{itemize}
  \item The probability that a recently published block will not belong to the
  longest branch is exactly $p$. This is the same as saying that the block
  will not be valid.
  \item The average rate at which the longest branch grows can be
  approximated by $p / \bar{T}$.
  \item The probability of a block with $k$ confirmations becoming invalid can
  be approximated by $p^k (1-p)^k$.
  \item The expected time for receiving one confirmation is $\bar{T}/p$.
\end{itemize}



